On the Decidability of Verification under Release/Acquire

The verification of concurrent programs under weak-memory models is a burgeoning effort, owing to the increasing adoption of weak memory in concurrent software and hardware. Release/Acquire has become the standard model for high-performance concurrent programming, adopted by common mainstream languages and computer architectures. In a surprising result, Abdulla et al. (PLDI'19) proved that reachability in this model is undecidable when programs have access to atomic Read-Modify-Write (RMW) operations. Moreover, undecidability holds even for executions with just 4 contexts, and is thus immune to underapproximations based on bounded context switching. The pure RMW-free case was left as a challenging question, and despite the attention it has received, it has remained open for the past seven years. In this paper, we settle the above open question by proving that reachability is undecidable even in the RMW-free fragment of Release/Acquire, thereby characterizing the simplest communication primitives that give rise to undecidability. Moreover, we prove that bounding both the number of context switches and the number of RMWs recovers decidability, thus fully characterizing the boundary of decidability along the dimensions of RMW-bounding and context-bounding.

==> macros.tex <==
\graphicspath{ {./} }

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\makeatletter
\renewcommand{\tagform@}[1]{\maketag@@@{\normalsize(#1)\@@italiccorr}}
\makeatother

\newcommand{\Paragraph}[1]{\smallskip\noindent{\bf #1}}
\newcommand{\SubParagraph}[1]{\smallskip\noindent{\em #1}}

\newlist{compactitem}{itemize}{3} % 3 is max-depth
\setlist[compactitem]{label={\Large \textbullet},nosep,leftmargin=*}
\crefname{compactitemi}{Item}{Items}

\newlist{compactenum}{enumerate}{3} % 3 is max-depth
\setlist[compactenum]{label=(\arabic*), nosep,leftmargin=*}
\crefname{compactenumi}{Item}{Items}

\makeatletter
\newcommand{\customlabel}[2]{%
   \protected@write \@auxout {}{\string \newlabel {#1}{{#2}{\thepage}{#2}{#1}{}} }%
   \hypertarget{#1}{#2}
}
\makeatother

\lstset{
    mathescape=true,
    basicstyle=\linespread{1.05}\tiny,
}

\sethlcolor{blue!10}
%\newcommand{\Revision}[1]{\hl{#1}}
\newcommand{\Revision}{}
\soulregister{\cite}{7}\soulregister{\ref}{7}\soulregister{\cref}{7}\soulregister{\Cref}{7}\soulregister{\circledsmall}{1}\soulregister{\squaredsmall}{1}

\def \xcolor {RoyalBlue}
\def \xpcolor {Blue}
\def \ycolor {RubineRed}
\def \ypcolor {Plum}
\def \zcolor {Bittersweet}
\def \zpcolor {Brown}
\def \lcolor {OliveGreen}

\colorlet{colorPO}{darkgray!80!black}
\colorlet{colorRF}{blue}
\colorlet{colorMO}{red!80!black}
\colorlet{colorHB}{green!40!black}


\usetikzlibrary{arrows,positioning}
\tikzset{
   >=stealth',
   main/.style={draw, rectangle, inner sep=4pt},
   every path/.style={>=stealth},
   rf/.style={->,color=colorRF,densely dashed, thick},
   hb/.style={->,color=colorHB,thick, thick},
   mo/.style={->,color=colorMO,densely dotted, very thick},
}

\newcommand*\circledsmall[1]{\tikz[baseline=(char.base)]{
  \node[shape=circle,draw=none,fill=orange!20!white,inner sep=0.7pt, solid] (char) {\textcolor{black}{\texttt{#1}}};}}

\newcommand*\squaredsmall[1]{\tikz[baseline=(char.base)]{
  \node[regular polygon, regular polygon sides=5,draw=none,fill=blue!15!white,inner sep=0.1pt, solid] (char) {\textcolor{black}{\small\texttt{#1}}};}}

\newcommand{\Nats}{\mathbb{N}}
\newcommand{\IntSet}[1]{[#1]}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\identity}[1]{[#1]}
\newcommand{\ov}{\overline}
\newcommand{\AnyValue}{*}
\def\Path{\mathcal{P}}

\newcommand{\LPath}[1]{\mathrel{\overset{\smash{\raisebox{-0.5ex}{\footnotesize $#1$}}}{\rightsquigarrow}}}
\newcommand{\LTo}[1]{\xrightarrow{\raisebox{-0.5ex}[0ex][0ex]{\footnotesize $#1$} } }
\newcommand{\nLTo}[1]{\not\xrightarrow{\raisebox{-0.5ex}[0ex][0ex]{\footnotesize \hspace{5pt}$#1$} } }
\newcommand{\LTransTo}[1]{\xhookrightarrow{\raisebox{-0.5ex}[0ex][0ex]{\footnotesize $#1$} } }

\newcommand{\NP}{\mathsf{NP}}
\newcommand{\NEXPTIME}{\mathsf{NEXP}}
\newcommand{\TWONEXPTIME}{\mathsf{2NEXP}}
\newcommand{\PSPACE}{\mathsf{PSPACE}}


\newcommand{\Prog}{\mathsf{Pseq}}
\newcommand{\ConcProg}{\mathsf{P}}
\newcommand{\numThreads}{{|\mathsf{Tid}|}}

\newcommand{\LTS}{\mathcal{A}}
\newcommand{\States}{\mathcal{Q}}
\newcommand{\Alphabet}{\Sigma}
\newcommand{\Trans}{\mathcal{T}}
\newcommand{\InitState}{\mathsf{q}_{\mathsf{in}}}
\newcommand{\FinalState}{\mathsf{q}_{\mathsf{fn}}}
\newcommand{\Word}[2]{\mathsf{Word}(#1,#2)}


\newcommand{\Events}{E}
\newcommand{\event}{e}
\newcommand{\op}{\mathsf{op}}
\newcommand{\tid}{\mathsf{tid}}
\newcommand{\id}{\mathsf{id}}
\newcommand{\llab}{\mathsf{lab}}
\newcommand{\lloc}{\mathsf{loc}}
\newcommand{\val}{\mathsf{val}}
\newcommand{\rd}{\mathtt{r}}
\newcommand{\wt}{\mathtt{w}}
\newcommand{\rmw}{\mathtt{rmw}}

\newcommand{\LabelDom}{\mathsf{Lab}}
\newcommand{\ValueDom}{\mathsf{Val}}
\newcommand{\LocationDom}{\mathsf{Loc}}
\newcommand{\ThreadDom}{\mathsf{Tid}}
\newcommand{\EventDom}{\mathsf{E}}
\newcommand{\ReadDom}{\mathsf{R}}
\newcommand{\WriteDom}{\mathsf{W}}
\newcommand{\RMWDom}{\mathsf{RMW}}

\newcommand{\In}{\mathsf{range}}
\newcommand{\EarliestWrite}{\mathsf{Ew}}
\newcommand{\LatestWrite}{\mathsf{Lw}}
\newcommand{\ch}{\mathsf{lt}}

\newcommand{\po}{\mathsf{\color{colorPO}po}}
\newcommand{\rf}{\mathsf{\color{colorRF}rf}}
\newcommand{\mo}{\mathsf{\color{colorMO}mo}}
\newcommand{\hb}{\mathsf{\color{colorHB}hb}}
\newcommand\locx[1]{{{#1}_{x}}}

\newcommand{\ExecutionGraphsOf}[2]{\llbracket{#1}\rrbracket}

\newcommand{\ramm}{\mathsf{RA}}
\newcommand{\tsomm}{\mathsf{TSO}}
\newcommand{\psomm}{\mathsf{PSO}}
\newcommand{\rdmamm}{\mathsf{RDMA}}


\newcommand{\PCPInstance}{\mathcal{I}}
\newcommand{\PCPAlphabet}{\Gamma}
\newcommand{\True}{\mathsf{T}}
\newcommand{\False}{\mathsf{F}}

% \betad: a beta with the height of an alpha
\ExplSyntaxOn
\cs_new:Npn \betad
  {{\mathchoice{\betadtext}{\betadtext}{\betadsub}{\betadsub}}}
\cs_new:Npn \betadtext
  { \group_begin:
    \exp_args:NNx\cs_set:Npn \next{\the\font}
    \hbox_set:Nn \l_tmpa_box {$\next\alpha$}
    \vbox_to_ht:nn {\box_ht:N \l_tmpa_box}
      { \hbox:n{$\next\beta$} \vss }
    \group_end: }

\cs_new:Npn \betadsub
  { \group_begin:
    \exp_args:NNx\cs_set:Npn \next{\the\font}
    \hbox_set:Nn \l_tmpa_box {$\next\alpha$}
    \hbox_set:Nn \l_tmpb_box {$\next\beta$}
    \box_scale:Nnn\l_tmpb_box {7/10}{7/10}
    \vbox_to_ht:nn {\box_ht:N \l_tmpa_box}
      { \box_use_drop:N\l_tmpb_box \vss }
    \box_clear:N\l_tmpa_box
    \group_end: }
\ExplSyntaxOff

\newcommand{\tx}{{c^x}}
\newcommand{\ty}{{c^y}}
\newcommand{\txp}{{c^{x'}}}
\newcommand{\typ}{{c^{y'}}}
\newcommand{\tax}{{g_{\alpha}^x}}
\newcommand{\taxp}{{g_{\alpha}^{x'}}}
\newcommand{\tay}{{g_{\alpha}^y}}
\newcommand{\tayp}{{g_{\alpha}^{y'}}}
\DeclareRobustCommand{\tbx}{{g_{\betad}^x}}
\DeclareRobustCommand{\tbxp}{{g_{\betad}^{x'}}}
\DeclareRobustCommand{\tby}{{g_{\betad}^y}}
\DeclareRobustCommand{\tbyp}{{g_{\betad}^{y'}}}
\newcommand{\tsnd}{{g^{u}}}
\newcommand{\tsndp}{{g^{u'}}}
\newcommand{\trcv}{{c^{u}}}
\newcommand{\trcvp}{{c^{u'}}}

\newcommand{\varix}{\textcolor{\xcolor}{x}}
\newcommand{\variy}{\textcolor{\ycolor}{y}}

\newcommand{\pc}{\mkern-6mu,}

\newcommand{\vxa}{\textcolor{\xcolor}{x_{\alpha}}}
\newcommand{\vxap}{\textcolor{\xpcolor}{x'_{\alpha}}}
\newcommand{\vxb}{\textcolor{\xcolor}{x_{\betad}}}
\newcommand{\vxbp}{\textcolor{\xpcolor}{x'_{\betad}}}
\newcommand{\vya}{\textcolor{\ycolor}{y_{\alpha}}}
\newcommand{\vyap}{\textcolor{\ypcolor}{y'_{\alpha}}}
\newcommand{\vyb}{\textcolor{\ycolor}{y_{\betad}}}
\newcommand{\vybp}{\textcolor{\ypcolor}{y'_{\betad}}}
\newcommand{\vch}{\textcolor{\xcolor}{u}}
\newcommand{\vchp}{\textcolor{\xpcolor}{u'}}
\newcommand{\vchz}{\textcolor{\zcolor}{z^{u,u'}}}
\newcommand{\vchzp}{\textcolor{\zpcolor}{z^{u'\pc u}}}
\newcommand{\vzax}{\textcolor{\zcolor}{z_{\alpha}^{x,x'}}}
\newcommand{\vzaxy}{\textcolor{\zcolor}{z_{\alpha}^{x,y}}}
\newcommand{\vzay}{\textcolor{\zcolor}{z_{\alpha}^{y,y'}}}
\newcommand{\vzaxp}{\textcolor{\zpcolor}{z_{\alpha}^{x'\pc x}}}
\newcommand{\vzaxyp}{\textcolor{\lcolor}{\ell_{\alpha}^{y,x}}}
\newcommand{\vzayp}{\textcolor{\zpcolor}{z_{\alpha}^{y'\pc y}}}
\newcommand{\vzbx}{\textcolor{\zcolor}{z_{\betad}^{x,x'}}}
\newcommand{\vzbxy}{\textcolor{\zcolor}{z_{\betad}^{x,y}}}
\newcommand{\vzby}{\textcolor{\zcolor}{z_{\betad}^{y,y'}}}
\newcommand{\vzbxp}{\textcolor{\zpcolor}{z_{\betad}^{x'\pc x}}}
\newcommand{\vzbxyp}{\textcolor{\lcolor}{\ell_{\betad}^{y,x}}}
\newcommand{\vzbyp}{\textcolor{\zpcolor}{z_{\betad}^{y'\pc y}}}

\newcommand{\ndet}[1]{\textcolor{black}{\textsc{NDet}(#1)}}
\newcommand{\firstit}{\ensuremath{\textcolor{black}{\textsc{First()}}}}
\newcommand{\vaux}{\ensuremath{\textcolor{black}{aux}}}
\newcommand{\vc}{\ensuremath{\textcolor{black}{cnt}}}
\newcommand{\vcy}{\ensuremath{\textcolor{black}{cnt_y}}}
\newcommand{\term}{\mathsf{term}}


\newcommand{\ctx}[1]{\mathsf{ctx}({#1})}
\newcommand{\LinearTrace}{\mathcal{T}}

\newcommand{\Summary}{\mathsf{Sum}}
\newcommand{\ContextId}{\mathsf{cid}}
\newcommand{\SummaryStates}{Q}
\newcommand{\SummaryLastValue}{\phi}
\newcommand{\SummaryExternalRf}{\mathsf{Erf}}
\newcommand{\SummaryDom}{\mathsf{Sums}}
\newcommand{\CSei}{\event_i}
\newcommand{\CSej}{\event_j}
\newcommand{\CSeb}{\event_b}
\newcommand{\CSwi}{\wt_i}
\newcommand{\CSwj}{\wt_j}
\newcommand{\CSrj}{\rd_j}
\newcommand{\CSrmwi}{\rmw_i}
\newcommand{\CSwp}{\wt'}
\newcommand{\CSwpp}{\wt''}
\newcommand{\CSid}{\mathsf{idx}}
\newcommand{\CSidp}{\mathsf{idx'}}

